Measurement of the branching fractions for Cabibbo-suppressed decays $D^{+}\to K^{+} K^{-}\pi^{+}\pi^{0}$ and $D_{(s)}^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0}$ at Belle

We present measurements of the branching fractions for the singly Cabibbo-suppressed decays $D^+\to K^{+}K^{-}\pi^{+}\pi^{0}$ and $D_s^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0}$, and the doubly Cabibbo-suppressed decay $D^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0}$, based on 980 ${\rm fb}^{-1}$ of data recorded by the Belle experiment at the KEKB $e^{+}e^{-}$ collider. We measure these modes relative to the Cabibbo-favored modes $D^{+}\to K^{-}\pi^{+}\pi^{+}\pi^{0}$ and $D_s^{+}\to K^{+}K^{-}\pi^{+}\pi^{0}$. Our results for the ratios of branching fractions are $B(D^{+}\to K^{+}K^{-}\pi^{+}\pi^{0})/B(D^{+}\to K^{-}\pi^{+}\pi^{+}\pi^{0}) = (11.32 \pm 0.13 \pm 0.26)\%$, $B(D^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0})/B(D^{+}\to K^{-}\pi^{+}\pi^{+}\pi^{0}) = (1.68 \pm 0.11\pm 0.03)\%$, and $B(D_s^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0})/B(D_s^{+}\to K^{+}K^{-}\pi^{+}\pi^{0}) = (17.13 \pm 0.62 \pm 0.51)\%$, where the uncertainties are statistical and systematic, respectively. The second value corresponds to $(5.83\pm 0.42)\times\tan^4\theta_C$, where $\theta_C$ is the Cabibbo angle; this value is larger than other measured ratios of branching fractions for a doubly Cabibbo-suppressed charm decay to a Cabibbo-favored decay. Multiplying these results by world average values for $B(D^{+}\to K^{-}\pi^{+}\pi^{+}\pi^{0})$ and $B(D_s^{+}\to K^{+}K^{-}\pi^{+}\pi^{0})$ yields $B(D^{+}\to K^{+}K^{-}\pi^{+}\pi^{0})= (7.08\pm 0.08\pm 0.16\pm 0.20)\times10^{-3}$, $B(D^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0})= (1.05\pm 0.07\pm 0.02\pm 0.03)\times10^{-3}$, and $B(D_s^{+}\to K^{+}\pi^{-}\pi^{+}\pi^{0}) = (9.44\pm 0.34\pm 0.28\pm 0.32)\times10^{-3}$, where the third uncertainty is due to the branching fraction of the normalization mode. The first two results are consistent with, but more precise than, the current world averages. The last result is the first measurement of this branching fraction.

==> alias.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II}

\newcommand{\CP}{\ensuremath{C\!P}\xspace}
%%\newcommand{\Acp}{\ensuremath{\mathcal{A}_{\CP}}\xspace}
\newcommand{\Acp}{\ensuremath{A_{\CP}}\xspace}
\newcommand{\Acpcor}{\ensuremath{\mathcal{A}^{cor}_{\CP}}\xspace}
%\newcommand{\Afb}{\ensuremath{\mathcal{A}_{FB}}\xspace}
\newcommand{\Afb}{\ensuremath{A_{\rm FB}}\xspace}

\newcommand{\BR}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\eff}{\ensuremath{\varepsilon}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pis  {\ensuremath{\pi^+_{s}}\xspace}
%\def\pips  {\ensuremath{\pi^+\mbox\,\rm{s}}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle\rm S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle\rm L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\D       {\ensuremath{D}\xspace}
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\part{\xspace}}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Dsp      {\ensuremath{D^+_s}\xspace}
\def\Dsm      {\ensuremath{D^-_s}\xspace}
\def\Dsstarp     {\ensuremath{D^{*+}_s}\xspace}
\def\Dsstarm     {\ensuremath{D^{*-}_s}\xspace}

\def\DDbar   {\ensuremath{\Dz{\text{-}}{\kern -0.16em \Dzb}}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}
\def\Bstbar  {\ensuremath{\Bbar{}^{(*)0}_s}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
%%%%\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

%\mathchardef\Deltares="7101
%\mathchardef\Xi="7104
%\mathchardef\Lambda="7103
%\mathchardef\Sigma="7106
%\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}






==> pub612.tex <==
%%% Paper:    D+ to K+ K- pi+ pi0, D(s)+ to K+ pi- pi+ pi0
%%% Journal:  Physical Review D
%%% Contacts: L. Li (lilk@ucmail.uc.edu)
%%%           A. Schwartz (alan.j.schwartz@uc.edu)
%%%           K. Kinoshita (kinoshky@ucmail.uc.edu)
%%%           E. Won (eunil@hep.korea.ac.kr)
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000}
\newcommand{\instEPFL}{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530}
\newcommand{\instIKERBASQUE}{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195}
\newcommand{\instKanagawa}{Kanagawa University, Yokohama 221-8686}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe}
\newcommand{\instKAU}{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich}
\newcommand{\instSMI}{Stefan Meyer Institute for Subatomic Physics, Vienna 1090}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506}
\newcommand{\instNCU}{National Central University, Chung-li 32054}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181}
\newcommand{\instNDU}{Nippon Dental University, Niigata 951-8580}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014}
\newcommand{\instPeking}{Peking University, Beijing 100871}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198}
\newcommand{\instRIKENBNL}{RIKEN BNL Research Center, Upton, New York 11973}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978}
\newcommand{\instToho}{Toho University, Funabashi 274-8510}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay}
\newcommand{\instBilbao}{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583}
\newcommand{\instUtkal}{Utkal University, Bhubaneswar 751004}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722}
\affiliation{\instGoettingen}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instPrague}
%%%\affiliation{\instChiba}
%%%\affiliation{\instChonnam}
\affiliation{\instCAU}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instEPFL}
\affiliation{\instJuelich}
%%%\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
%%%\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHiroshima}
\affiliation{\instIKERBASQUE}
\affiliation{\instNapoliINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instISU}
\affiliation{\instJAEA}
%%%\affiliation{\instKanagawa}
\affiliation{\instKarlsruhe}
\affiliation{\instKAU}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyungpook}
%%%\affiliation{\instLNNU}
%%%\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
%%%\affiliation{\instSMI}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
%%%\affiliation{\instNagoyaKMI}
\affiliation{\instNaraWu}
\affiliation{\instNCU}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNDU}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKENBNL}
%%%\affiliation{\instSeoul}
\affiliation{\instSPU}
%%%\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
\affiliation{\instTelAviv}
%%%\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
%%%\affiliation{\instTokyoMetropolitan}
\affiliation{\instNapoliUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instIJCLab}
\affiliation{\instBilbao}
\affiliation{\instBonn}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
%%%\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSydney}
\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
%%%\affiliation{\instUtkal}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYonsei}

  \author{L.~K.~Li}\affiliation{\instCincinnati} % Cincinnati
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % Cincinnati
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % Cincinnati
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % Korea

% \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Adamczyk}\affiliation{\instKrakow} % Krakow
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % Korea
  \author{H.~Aihara}\affiliation{\instUTokyo} % Tokyo
  \author{S.~Al~Said}\affiliation{\instTabuk}\affiliation{\instKAU} % Tabuk
  \author{D.~M.~Asner}\affiliation{\instBNL} % BNL
  \author{H.~Atmacan}\affiliation{\instCincinnati} % Cincinnati
  \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{T.~Aushev}\affiliation{\instHSE} % HSE
  \author{R.~Ayad}\affiliation{\instTabuk} % Tabuk
% \author{T.~Aziz}\affiliation{\instTata} % Tata
  \author{V.~Babu}\affiliation{\instDESY} % DESY
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % IITB
% \author{A.~M.~Bakich}\affiliation{\instSydney} % Sydney
% \author{Y.~Ban}\affiliation{\instPeking} % Peking
% \author{E.~Barberio}\affiliation{\instMelbourne} % Melbourne
% \author{M.~Barrett}\affiliation{\instKEK} % KEK
% \author{M.~Bauer}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{P.~Behera}\affiliation{\instIITMadras} % IITM
  \author{K.~Belous}\affiliation{\instIHEPRussia} % Protvino
  \author{J.~Bennett}\affiliation{\instMississippi} % Mississippi
% \author{F.~Bernlochner}\affiliation{\instBonn} % Bonn
  \author{M.~Bessner}\affiliation{\instHawaii} % Hawaii
% \author{D.~Besson}\affiliation{\instMEPhI} % MEPhI
  \author{V.~Bhardwaj}\affiliation{\instIISER} % IISERM
% \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % IITG
  \author{T.~Bilka}\affiliation{\instPrague} % Charles
% \author{S.~Bilokin}\affiliation{\instLMU} % LMU
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{D.~Bodrov}\affiliation{\instHSE} % HSE
% \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{G.~Bonvicini}\affiliation{\instWayneState} % WayneState
  \author{J.~Borah}\affiliation{\instIITGuwahati} % IITG
  \author{A.~Bozek}\affiliation{\instKrakow} % Krakow
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % RomaTre
  \author{T.~E.~Browder}\affiliation{\instHawaii} % Hawaii
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % RomaTre
  \author{M.~Campajola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
% \author{L.~Cao}\affiliation{\instDESY} % DESY
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % Charles
% \author{M.-C.~Chang}\affiliation{\instFuJen} % FuJen
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{V.~Chekelian}\affiliation{\instMPP} % MPI
  \author{A.~Chen}\affiliation{\instNCU} % NCU
% \author{C.~Chen}\affiliation{\instISU} % ISU
% \author{Y.~Chen}\affiliation{\instUSTC} % USTC
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % Taiwan
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % Hanyang
% \author{K.~Chilikin}\affiliation{\instBINP} % BINP
  \author{H.~E.~Cho}\affiliation{\instHanyang} % Hanyang
  \author{K.~Cho}\affiliation{\instKISTI} % KISTI
  \author{S.-J.~Cho}\affiliation{\instYonsei} % Yonsei
  \author{S.-K.~Choi}\affiliation{\instCAU} % CAU
  \author{Y.~Choi}\affiliation{\instSKKU} % Sungkyunkwan
  \author{S.~Choudhury}\affiliation{\instISU} % ISU
  \author{D.~Cinabro}\affiliation{\instWayneState} % WayneState
% \author{J.~Cochran}\affiliation{\instISU} % ISU
  \author{S.~Cunliffe}\affiliation{\instDESY} % DESY
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % TMU
  \author{S.~Das}\affiliation{\instMNITJaipur} % MNIT
  \author{N.~Dash}\affiliation{\instIITMadras} % IITM
% \author{G.~de~Marino}\affiliation{\instIJCLab} % IJCLab
  \author{G.~De~Nardo}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % RomaTre
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % IITH
  \author{F.~Di~Capua}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
% \author{J.~Dingfelder}\affiliation{\instBonn} % Bonn
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % Charles
  \author{T.~V.~Dong}\affiliation{\instITAR} % DuyTan
  \author{D.~Dossett}\affiliation{\instMelbourne} % Melbourne
% \author{S.~Dubey}\affiliation{\instHawaii} % Hawaii
% \author{P.~Ecker}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{M.~Feindt}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{T.~Ferber}\affiliation{\instDESY} % DESY
% \author{D.~Ferlewicz}\affiliation{\instMelbourne} % Melbourne
  \author{A.~Frey}\affiliation{\instGoettingen} % Goettingen
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % PNNL
  \author{R.~Garg}\affiliation{\instPanjab} % Panjab
  \author{V.~Gaur}\affiliation{\instVPI}\affiliation{\instKEK} % VPI
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Giri}\affiliation{\instIITHyderabad} % IITH
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{G.~Gong}\affiliation{\instUSTC} % USTC
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % RomaTre
  \author{D.~Greenwald}\affiliation{\instTUM} % TUM
  \author{T.~Gu}\affiliation{\instPittsburgh} % Pittsburgh
  \author{Y.~Guan}\affiliation{\instCincinnati} % Cincinnati
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % PNNL
% \author{S.~Halder}\affiliation{\instTata} % Tata
% \author{K.~Hara}\affiliation{\instKEK} % KEK
% \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{O.~Hartbrich}\affiliation{\instHawaii} % Hawaii
  \author{K.~Hayasaka}\affiliation{\instNiigata} % Niigata
  \author{H.~Hayashii}\affiliation{\instNaraWu} % Nara
% \author{S.~Hazra}\affiliation{\instTata} % Tata
% \author{M.~T.~Hedges}\affiliation{\instHawaii} % Hawaii
  \author{D.~Herrmann}\affiliation{\instWayneState} % WayneState
% \author{M.~Hernandez~Villanueva}\affiliation{\instDESY} % DESY
% \author{T.~Higuchi}\affiliation{\instIPMU} % IPMU
  \author{W.-S.~Hou}\affiliation{\instNTUTaiwan} % Taiwan
  \author{C.-L.~Hsu}\affiliation{\instSydney} % Sydney
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{T.~Iijima}\affiliation{\instNagoyaKMI}\affiliation{\instNagoya} % Nagoya
  \author{K.~Inami}\affiliation{\instNagoya} % Nagoya
% \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % Vienna
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{Y.~Iwasaki}\affiliation{\instKEK} % KEK
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % TMU
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % Indiana
% \author{E.-J.~Jang}\affiliation{\instGyeongsang} % Gyeongsang
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % Kyungpook
  \author{S.~Jia}\affiliation{\instFudan} % Fudan
  \author{Y.~Jin}\affiliation{\instUTokyo} % Tokyo
% \author{K.~K.~Joo}\affiliation{\instChonnam} % Chonnam
% \author{J.~Kahn}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % TMU
  \author{D.~Kalita}\affiliation{\instIITGuwahati} % IITG
  \author{A.~B.~Kaliyar}\affiliation{\instTata} % Tata
  \author{K.~H.~Kang}\affiliation{\instIPMU} % IPMU
% \author{S.~Kang}\affiliation{\instISU} % ISU
% \author{P.~Kapusta}\affiliation{\instKrakow} % Krakow
% \author{G.~Karyan}\affiliation{\instDESY} % DESY
% \author{Y.~Kato}\affiliation{\instNagoya} % Nagoya
% \author{H.~Kawai}\affiliation{\instChiba} % Chiba
  \author{T.~Kawasaki}\affiliation{\instKitasato} % Kitasato
% \author{H.~Kichimi}\affiliation{\instKEK} % KEK
  \author{C.~Kiesling}\affiliation{\instMPP} % MPI
  \author{C.~H.~Kim}\affiliation{\instHanyang} % Hanyang
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % Soongsil
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % Kyungpook
  \author{K.-H.~Kim}\affiliation{\instYonsei} % Yonsei
  \author{K.~T.~Kim}\affiliation{\instKoreaUnivKU} % Korea
% \author{S.~K.~Kim}\affiliation{\instSeoul} % Seoul
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % Korea
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % Yonsei
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % VPI
% \author{H.~Kindo}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{C.~Kleinwort}\affiliation{\instDESY} % DESY
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % Charles
% \author{I.~Komarov}\affiliation{\instDESY} % DESY
  \author{T.~Konno}\affiliation{\instKitasato} % Kitasato
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{R.~Kroeger}\affiliation{\instMississippi} % Mississippi
% \author{J.-F.~Krohn}\affiliation{\instMelbourne} % Melbourne
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{T.~Kuhr}\affiliation{\instLMU} % LMU
  \author{M.~Kumar}\affiliation{\instMNITJaipur} % MNIT
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % Punjab
  \author{K.~Kumara}\affiliation{\instMississippi} % Mississippi
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % TMU
% \author{E.~Kurihara}\affiliation{\instChiba} % Chiba
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % Charles
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % Yonsei
  \author{Y.-T.~Lai}\affiliation{\instIPMU} % IPMU
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % MNIT
  \author{T.~Lam}\affiliation{\instVPI} % VPI
% \author{J.~S.~Lange}\affiliation{\instGiessen} % Giessen
  \author{M.~Laurenza}\affiliation{\instRomaTreINFN}\affiliation{\instRomaTreUNIV} % RomaTre
% \author{I.~S.~Lee}\affiliation{\instHanyang} % Hanyang
% \author{J.~K.~Lee}\affiliation{\instSeoul} % Seoul
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % Kyungpook
% \author{D.~Levit}\affiliation{\instTUM} % TUM
% \author{P.~Lewis}\affiliation{\instBonn} % Bonn
% \author{C.~H.~Li}\affiliation{\instLNNU} % LNNU
  \author{J.~Li}\affiliation{\instKyungpook} % Kyungpook
% \author{S.~X.~Li}\affiliation{\instFudan} % Fudan
  \author{Y.~Li}\affiliation{\instFudan} % Fudan
  \author{Y.~B.~Li}\affiliation{\instFudan} % Fudan
% \author{Z.~Li}\affiliation{\instUSTC} % USTC
  \author{L.~Li~Gioi}\affiliation{\instMPP} % MPI
  \author{J.~Libby}\affiliation{\instIITMadras} % IITM
  \author{K.~Lieret}\affiliation{\instLMU} % LMU
% \author{Z.~Liptak}\affiliation{\instHiroshima} % Hiroshima
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % WayneState
% \author{T.~Luo}\affiliation{\instFudan} % Fudan
% \author{J.~MacNaughton}\affiliation{\instUOM} % NPC
  \author{A.~Martini}\affiliation{\instDESY} % DESY
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % NPC
  \author{T.~Matsuda}\affiliation{\instUOM} % NPC
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % IITG
  \author{F.~Meier}\affiliation{\instDuke} % Duke
  \author{M.~Merola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % Nara
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Miyata}\affiliation{\instNiigata} % Niigata
  \author{R.~Mizuk}\affiliation{\instHSE} % HSE
  \author{G.~B.~Mohanty}\affiliation{\instTata} % Tata
  \author{H.~K.~Moon}\affiliation{\instKoreaUnivKU} % Korea
% \author{T.~J.~Moon}\affiliation{\instSeoul} % Seoul
% \author{H.-G.~Moser}\affiliation{\instMPP} % MPI
% \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % Vienna
% \author{T.~M\"uller}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{R.~Mussa}\affiliation{\instTorinoINFN} % Torino
% \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~R.~Nakamura}\affiliation{\instKEK} % KEK
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{T.~Nakano}\affiliation{\instRCNP} % NPC
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % Taiwan
% \author{D.~Narwal}\affiliation{\instIITGuwahati} % IITG
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % Krakow
  \author{A.~Natochii}\affiliation{\instHawaii} % Hawaii
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % IITH
  \author{M.~Nayak}\affiliation{\instTelAviv} % TelAviv
% \author{C.~Niebuhr}\affiliation{\instDESY} % DESY
% \author{M.~Niiyama}\affiliation{\instKSU} % NPC
  \author{N.~K.~Nisar}\affiliation{\instBNL} % BNL
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Nishimura}\affiliation{\instHawaii} % Hawaii
% \author{K.~Ogawa}\affiliation{\instNiigata} % Niigata
% \author{S.~Ogawa}\affiliation{\instToho} % Toho
% \author{S.~Okuno}\affiliation{\instKanagawa} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{\instCAU} % CAU
  \author{H.~Ono}\affiliation{\instNDU}\affiliation{\instNiigata} % NihonDental
% \author{Y.~Onuki}\affiliation{\instUTokyo} % Tokyo
  \author{P.~Oskin}\affiliation{\instIJCLab} % IJCLab
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{P.~Pakhlov}\affiliation{\instHSE} % HSE
  \author{G.~Pakhlova}\affiliation{\instHSE} % HSE
% \author{T.~Pang}\affiliation{\instPittsburgh} % Pittsburgh
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % Napoli
  \author{H.~Park}\affiliation{\instKyungpook} % Kyungpook
  \author{S.-H.~Park}\affiliation{\instKEK} % KEK
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % RomaTre
  \author{S.~Patra}\affiliation{\instIISER} % IISERM
  \author{S.~Paul}\affiliation{\instTUM}\affiliation{\instMPP} % TUM
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % Luther
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % VPI
  \author{T.~Podobnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Popov}\affiliation{\instHSE} % HSE
% \author{S.~Prell}\affiliation{\instISU} % ISU
  \author{E.~Prencipe}\affiliation{\instJuelich} % Juelich
  \author{M.~T.~Prim}\affiliation{\instBonn} % Bonn
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % OIST
% \author{A.~Rabusov}\affiliation{\instTUM} % TUM
% \author{M.~Ritter}\affiliation{\instLMU} % LMU
% \author{M.~R\"{o}hrken}\affiliation{\instDESY} % DESY
  \author{A.~Rostomyan}\affiliation{\instDESY} % DESY
  \author{N.~Rout}\affiliation{\instIITMadras} % IITM
% \author{M.~Rozanska}\affiliation{\instKrakow} % Krakow
  \author{G.~Russo}\affiliation{\instNapoliUNIV} % Napoli
  \author{D.~Sahoo}\affiliation{\instISU} % ISU
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{M.~Salehi}\affiliation{\instMalaya}\affiliation{\instLMU} % Malaya
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % IITH
  \author{A.~Sangal}\affiliation{\instCincinnati} % Cincinnati
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{T.~Sanuki}\affiliation{\instTohoku} % Tohoku
  \author{V.~Savinov}\affiliation{\instPittsburgh} % Pittsburgh
% \author{P.~Schmolz}\affiliation{\instLMU} % LMU
% \author{O.~Schneider}\affiliation{\instEPFL} % Lausanne
  \author{G.~Schnell}\affiliation{\instBilbao}\affiliation{\instIKERBASQUE} % Bilbao
% \author{M.~Schram}\affiliation{\instPNNL} % PNNL
  \author{J.~Schueler}\affiliation{\instHawaii} % Hawaii
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % Vienna
% \author{B.~Schwenker}\affiliation{\instGoettingen} % Goettingen
% \author{R.~Seidl}\affiliation{\instRIKENBNL} % RIKEN
  \author{Y.~Seino}\affiliation{\instNiigata} % Niigata
  \author{K.~Senyo}\affiliation{\instYamagata} % Yamagata
% \author{O.~Seon}\affiliation{\instNagoya} % Nagoya
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % Melbourne
  \author{M.~Shapkin}\affiliation{\instIHEPRussia} % Protvino
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % MNIT
% \author{V.~Shebalin}\affiliation{\instHawaii} % Hawaii
% \author{C.~P.~Shen}\affiliation{\instFudan} % Fudan
% \author{H.~Shibuya}\affiliation{\instToho} % Toho
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % Taiwan
% \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{A.~Sibidanov}\affiliation{\instSydney} % Sydney
  \author{F.~Simon}\affiliation{\instMPP} % MPI
  \author{J.~B.~Singh}\affiliation{\instPanjab}\affiliation{\instUPES} % Panjab
% \author{R.~Sinha}\affiliation{\instChennai} % IMSC
% \author{K.~Smith}\affiliation{\instMelbourne} % Melbourne
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % Protvino
% \author{Y.~Soloviev}\affiliation{\instDESY} % DESY
  \author{E.~Solovieva}\affiliation{\instBINP} % BINP
% \author{S.~Stani\v{c}}\affiliation{\instNovaGorica} % NovaGorica
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % VPI
% \author{J.~F.~Strube}\affiliation{\instPNNL} % PNNL
% \author{J.~Stypula}\affiliation{\instKrakow} % Krakow
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % NPC
% \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % TMU
% \author{W.~Sutcliffe}\affiliation{\instBonn} % Bonn
% \author{S.~Y.~Suzuki}\affiliation{\instKEK} % KEK
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % NPC
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % Torino
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{K.~Tanida}\affiliation{\instJAEA} % NPC
% \author{N.~Taniguchi}\affiliation{\instKEK} % KEK
% \author{Y.~Tao}\affiliation{\instFlorida} % Florida
% \author{G.~N.~Taylor}\affiliation{\instMelbourne} % Melbourne
  \author{F.~Tenchini}\affiliation{\instDESY} % DESY
% \author{Y.~Teramoto}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{A.~Thampi}\affiliation{\instJuelich} % Juelich
% \author{R.~Tiwary}\affiliation{\instTata} % Tata
% \author{K.~Trabelsi}\affiliation{\instIJCLab} % IJCLab
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{M.~Uchida}\affiliation{\instTitech} % NPC
% \author{I.~Ueda}\affiliation{\instKEK} % KEK
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{T.~Uglov}\affiliation{\instHSE} % HSE
% \author{Y.~Unno}\affiliation{\instHanyang} % Hanyang
  \author{K.~Uno}\affiliation{\instNiigata} % Niigata
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{P.~Urquijo}\affiliation{\instMelbourne} % Melbourne
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{S.~E.~Vahsen}\affiliation{\instHawaii} % Hawaii
  \author{R.~van~Tonder}\affiliation{\instBonn} % Bonn
  \author{G.~Varner}\affiliation{\instHawaii} % Hawaii
  \author{K.~E.~Varvell}\affiliation{\instSydney} % Sydney
% \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{V.~Vorobyev}\affiliation{\instBINP} % BINP
  \author{A.~Vossen}\affiliation{\instDuke} % Duke
  \author{E.~Waheed}\affiliation{\instKEK} % KEK
% \author{B.~Wang}\affiliation{\instMPP} % MPI
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % NUU
% \author{D.~Wang}\affiliation{\instFlorida} % Florida
  \author{E.~Wang}\affiliation{\instPittsburgh} % Pittsburgh
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % Taiwan
  \author{X.~L.~Wang}\affiliation{\instFudan} % Fudan
% \author{M.~Watanabe}\affiliation{\instNiigata} % Niigata
% \author{Y.~Watanabe}\affiliation{\instKanagawa} % Kanagawa
  \author{S.~Watanuki}\affiliation{\instYonsei} % Yonsei
% \author{S.~Wehle}\affiliation{\instDESY} % DESY
  \author{O.~Werbycka}\affiliation{\instKrakow} % Krakow
% \author{E.~Widmann}\affiliation{\instSMI} % Vienna
  \author{J.~Wiechczynski}\affiliation{\instKrakow} % Krakow
% \author{X.~Xu}\affiliation{\instSoochow} % Soochow
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % Sydney
% \author{S.~Yamada}\affiliation{\instKEK} % KEK
% \author{H.~Yamamoto}\affiliation{\instTohoku} % Tohoku
  \author{W.~Yan}\affiliation{\instUSTC} % USTC
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % Korea
  \author{H.~Ye}\affiliation{\instDESY} % DESY
  \author{J.~Yelton}\affiliation{\instFlorida} % Florida
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % Korea
% \author{Y.~Yook}\affiliation{\instYonsei} % Yonsei
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % IHEP
% \author{Y.~Yusa}\affiliation{\instNiigata} % Niigata
% \author{Y.~Zhai}\affiliation{\instISU} % ISU
% \author{J.~Zhang}\affiliation{\instIHEPChina} % IHEP
  \author{Z.~P.~Zhang}\affiliation{\instUSTC} % USTC
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{V.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
\collaboration{The Belle Collaboration}


==> pub612_v0.tex <==
%%% Paper:    D+ to K+ K- pi+ pi0, D(s)+ to K+ pi- pi+ pi0
%%% Journal:  Physical Review D
%%% Contacts: L. Li (lilk@ucmail.uc.edu)
%%%           A. Schwartz (alan.j.schwartz@uc.edu)
%%%           K. Kinoshita (kinoshky@ucmail.uc.edu)
%%%           E. Won (eunil@hep.korea.ac.kr)
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
\affiliation{Department of Physics, University of the Basque Country UPV/EHU, 48080 Bilbao}
\affiliation{University of Bonn, 53115 Bonn}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}
\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague}
%%%\affiliation{Chiba University, Chiba 263-8522}
%%%\affiliation{Chonnam National University, Gwangju 61186}
\affiliation{Chung-Ang University, Seoul 06974}
\affiliation{University of Cincinnati, Cincinnati, Ohio 45221}
\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg}
\affiliation{Duke University, Durham, North Carolina 27708}
\affiliation{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000}
\affiliation{University of Florida, Gainesville, Florida 32611}
%%%\affiliation{Department of Physics, Fu Jen Catholic University, Taipei 24205}
\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443}
%%%\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en}
\affiliation{Gifu University, Gifu 501-1193}
\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen}
\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193}
%%%\affiliation{Gyeongsang National University, Jinju 52828}
\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763}
\affiliation{University of Hawaii, Honolulu, Hawaii 96822}
\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\affiliation{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\affiliation{National Research University Higher School of Economics, Moscow 101000}
\affiliation{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich}
%%%\affiliation{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530}
\affiliation{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao}
\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306}
\affiliation{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007}
\affiliation{Indian Institute of Technology Guwahati, Assam 781039}
\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285}
\affiliation{Indian Institute of Technology Madras, Chennai 600036}
\affiliation{Indiana University, Bloomington, Indiana 47408}
\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049}
\affiliation{Institute of High Energy Physics, Vienna 1050}
\affiliation{Institute for High Energy Physics, Protvino 142281}
%%%\affiliation{Institute of Mathematical Sciences, Chennai 600113}
\affiliation{INFN - Sezione di Napoli, I-80126 Napoli}
\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma}
\affiliation{INFN - Sezione di Torino, I-10125 Torino}
\affiliation{Iowa State University, Ames, Iowa 50011}
\affiliation{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195}
\affiliation{J. Stefan Institute, 1000 Ljubljana}
%%%\affiliation{Kanagawa University, Yokohama 221-8686}
\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583}
%%%\affiliation{King Abdulaziz City for Science and Technology, Riyadh 11442}
\affiliation{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589}
\affiliation{Kitasato University, Sagamihara 252-0373}
\affiliation{Korea Institute of Science and Technology Information, Daejeon 34141}
\affiliation{Korea University, Seoul 02841}
%%%\affiliation{Kyoto Sangyo University, Kyoto 603-8555}
\affiliation{Kyungpook National University, Daegu 41566}
%%%\affiliation{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay}
%%%\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015}
\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}
%%%\affiliation{Liaoning Normal University, Dalian 116029}
\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}
\affiliation{Ludwig Maximilians University, 80539 Munich}
\affiliation{Luther College, Decorah, Iowa 52101}
\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017}
%%%\affiliation{University of Malaya, 50603 Kuala Lumpur}
\affiliation{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen}
\affiliation{School of Physics, University of Melbourne, Victoria 3010}
\affiliation{University of Mississippi, University, Mississippi 38677}
\affiliation{University of Miyazaki, Miyazaki 889-2192}
%%%\affiliation{Moscow Physical Engineering Institute, Moscow 115409}
\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602}
%%%\affiliation{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}
\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli}
\affiliation{Nara Women's University, Nara 630-8506}
\affiliation{National Central University, Chung-li 32054}
%%%\affiliation{National United University, Miao Li 36003}
\affiliation{Department of Physics, National Taiwan University, Taipei 10617}
\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342}
\affiliation{Nippon Dental University, Niigata 951-8580}
\affiliation{Niigata University, Niigata 950-2181}
%%%\affiliation{University of Nova Gorica, 5000 Nova Gorica}
\affiliation{Novosibirsk State University, Novosibirsk 630090}
%%%\affiliation{Okinawa Institute of Science and Technology, Okinawa 904-0495}
\affiliation{Osaka City University, Osaka 558-8585}
\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352}
\affiliation{Panjab University, Chandigarh 160014}
%%%\affiliation{Peking University, Beijing 100871}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\affiliation{Punjab Agricultural University, Ludhiana 141004}
%%%\affiliation{Research Center for Electron Photon Science, Tohoku University, Sendai 980-8578}
\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047}
\affiliation{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198}
%%%\affiliation{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198}
%%%\affiliation{RIKEN BNL Research Center, Upton, New York 11973}
\affiliation{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma}
\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026}
%%%\affiliation{Seoul National University, Seoul 08826}
\affiliation{Showa Pharmaceutical University, Tokyo 194-8543}
%%%\affiliation{Soochow University, Suzhou 215006}
\affiliation{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978}
%%%\affiliation{University of South Carolina, Columbia, South Carolina 29208}
%%%\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090}
\affiliation{Sungkyunkwan University, Suwon 16419}
\affiliation{School of Physics, University of Sydney, New South Wales 2006}
\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}
\affiliation{Tata Institute of Fundamental Research, Mumbai 400005}
%%%\affiliation{Excellence Cluster Universe, Technische Universit\"at M\"unchen, 85748 Garching}
\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching}
\affiliation{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978}
%%%\affiliation{Toho University, Funabashi 274-8510}
%%%\affiliation{Department of Physics, Tohoku University, Sendai 980-8578}
\affiliation{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}
\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033}
\affiliation{Tokyo Institute of Technology, Tokyo 152-8550}
%%%\affiliation{Tokyo Metropolitan University, Tokyo 192-0397}
%%%\affiliation{Utkal University, Bhubaneswar 751004}
\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\affiliation{Wayne State University, Detroit, Michigan 48202}
\affiliation{Yamagata University, Yamagata 990-8560}
\affiliation{Yonsei University, Seoul 03722}

  \author{L.~K.~Li}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{A.~J.~Schwartz}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati  
  \author{K.~Kinoshita}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
 \author{E.~Won}\affiliation{Korea University, Seoul 02841} % Korea

% \author{I.~Adachi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{K.~Adamczyk}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{J.~K.~Ahn}\affiliation{Korea University, Seoul 02841} % Korea
  \author{H.~Aihara}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
  \author{S.~Al~Said}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}\affiliation{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589} % Tabuk
  \author{D.~M.~Asner}\affiliation{Brookhaven National Laboratory, Upton, New York 11973} % BNL
  \author{H.~Atmacan}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{V.~Aulchenko}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{T.~Aushev}\affiliation{National Research University Higher School of Economics, Moscow 101000} % HSE
  \author{R.~Ayad}\affiliation{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451} % Tabuk
% \author{T.~Aziz}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
  \author{V.~Babu}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{S.~Bahinipati}\affiliation{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007} % IITB
% \author{A.~M.~Bakich}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{Y.~Ban}\affiliation{Peking University, Beijing 100871} % Peking
% \author{E.~Barberio}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{M.~Barrett}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{M.~Bauer}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{P.~Behera}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
  \author{K.~Belous}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
  \author{J.~Bennett}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{F.~Bernlochner}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{M.~Bessner}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{D.~Besson}\affiliation{Moscow Physical Engineering Institute, Moscow 115409} % MEPhI
  \author{V.~Bhardwaj}\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306} % IISERM
% \author{B.~Bhuyan}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
  \author{T.~Bilka}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{S.~Bilokin}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
  \author{A.~Bobrov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{D.~Bodrov}\affiliation{National Research University Higher School of Economics, Moscow 101000}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % HSE
% \author{A.~Bondar}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{G.~Bonvicini}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
  \author{J.~Borah}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
  \author{A.~Bozek}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{M.~Bra\v{c}ko}\affiliation{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{P.~Branchini}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma} % RomaTre
% \author{N.~Braun}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{T.~E.~Browder}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{A.~Budano}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma} % RomaTre
  \author{M.~Campajola}\affiliation{INFN - Sezione di Napoli, I-80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli} % Napoli
% \author{L.~Cao}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{D.~\v{C}ervenkov}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{M.-C.~Chang}\affiliation{Department of Physics, Fu Jen Catholic University, Taipei 24205} % FuJen
  \author{P.~Chang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{V.~Chekelian}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{A.~Chen}\affiliation{National Central University, Chung-li 32054} % NCU
% \author{C.~Chen}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
% \author{Y.~Chen}\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026} % USTC
% \author{Y.-T.~Chen}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
  \author{B.~G.~Cheon}\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763} % Hanyang
% \author{K.~Chilikin}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
  \author{H.~E.~Cho}\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763} % Hanyang
  \author{K.~Cho}\affiliation{Korea Institute of Science and Technology Information, Daejeon 34141} % KISTI
  \author{S.-J.~Cho}\affiliation{Yonsei University, Seoul 03722} % Yonsei
  \author{S.-K.~Choi}\affiliation{Chung-Ang University, Seoul 06974} % CAU
  \author{Y.~Choi}\affiliation{Sungkyunkwan University, Suwon 16419} % Sungkyunkwan
  \author{S.~Choudhury}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
  \author{D.~Cinabro}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
% \author{J.~Cochran}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
  \author{S.~Cunliffe}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{T.~Czank}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
  \author{S.~Das}\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017} % MNIT
  \author{N.~Dash}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
% \author{G.~de~Marino}\affiliation{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay} % IJCLab
  \author{G.~De~Nardo}\affiliation{INFN - Sezione di Napoli, I-80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli} % Napoli
  \author{G.~De~Pietro}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma} % RomaTre
  \author{R.~Dhamija}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{F.~Di~Capua}\affiliation{INFN - Sezione di Napoli, I-80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli} % Napoli
% \author{J.~Dingfelder}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{Z.~Dole\v{z}al}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
  \author{T.~V.~Dong}\affiliation{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000} % DuyTan
  \author{D.~Dossett}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
% \author{S.~Dubey}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{P.~Ecker}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{D.~Epifanov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{M.~Feindt}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{T.~Ferber}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{D.~Ferlewicz}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{A.~Frey}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
  \author{B.~G.~Fulsom}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
  \author{R.~Garg}\affiliation{Panjab University, Chandigarh 160014} % Panjab
  \author{V.~Gaur}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{N.~Gabyshev}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{A.~Garmash}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{A.~Giri}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{P.~Goldenzweig}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{B.~Golob}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{G.~Gong}\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026} % USTC
  \author{E.~Graziani}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma} % RomaTre
  \author{D.~Greenwald}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
  \author{T.~Gu}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
  \author{Y.~Guan}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{K.~Gudkova}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{C.~Hadjivasiliou}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{S.~Halder}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{K.~Hara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{T.~Hara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{O.~Hartbrich}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{K.~Hayasaka}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{H.~Hayashii}\affiliation{Nara Women's University, Nara 630-8506} % Nara
% \author{S.~Hazra}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{M.~T.~Hedges}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{D.~Herrmann}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
% \author{M.~Hernandez~Villanueva}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{T.~Higuchi}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{S.~Hirose}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{W.-S.~Hou}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
  \author{C.-L.~Hsu}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{K.~Huang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{T.~Iijima}\affiliation{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
  \author{K.~Inami}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{G.~Inguglia}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
  \author{A.~Ishikawa}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{R.~Itoh}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{M.~Iwasaki}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
% \author{Y.~Iwasaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{S.~Iwata}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
  \author{W.~W.~Jacobs}\affiliation{Indiana University, Bloomington, Indiana 47408} % Indiana
% \author{I.~Jaegle}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
% \author{E.-J.~Jang}\affiliation{Gyeongsang National University, Jinju 52828} % Gyeongsang
% \author{H.~B.~Jeon}\affiliation{Kyungpook National University, Daegu 41566} % Kyungpook
  \author{S.~Jia}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
  \author{Y.~Jin}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
% \author{C.~W.~Joo}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{K.~K.~Joo}\affiliation{Chonnam National University, Gwangju 61186} % Chonnam
% \author{J.~Kahn}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{H.~Kakuno}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
  \author{D.~Kalita}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
  \author{A.~B.~Kaliyar}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
  \author{K.~H.~Kang}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{S.~Kang}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
% \author{P.~Kapusta}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{G.~Karyan}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{Y.~Kato}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{H.~Kawai}\affiliation{Chiba University, Chiba 263-8522} % Chiba
  \author{T.~Kawasaki}\affiliation{Kitasato University, Sagamihara 252-0373} % Kitasato
% \author{H.~Kichimi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{C.~Kiesling}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{B.~H.~Kim}\affiliation{Seoul National University, Seoul 08826} % Seoul
  \author{C.~H.~Kim}\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763} % Hanyang
  \author{D.~Y.~Kim}\affiliation{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978} % Soongsil
% \author{H.~J.~Kim}\affiliation{Kyungpook National University, Daegu 41566} % Kyungpook
  \author{K.-H.~Kim}\affiliation{Yonsei University, Seoul 03722} % Yonsei
  \author{K.~T.~Kim}\affiliation{Korea University, Seoul 02841} % Korea
% \author{S.~H.~Kim}\affiliation{Seoul National University, Seoul 08826} % Seoul
% \author{S.~K.~Kim}\affiliation{Seoul National University, Seoul 08826} % Seoul
% \author{Y.~J.~Kim}\affiliation{Korea University, Seoul 02841} % Korea
  \author{Y.-K.~Kim}\affiliation{Yonsei University, Seoul 03722} % Yonsei
% \author{T.~D.~Kimmel}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{H.~Kindo}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
%  \author{K.~Kinoshita}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{C.~Kleinwort}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{P.~Kody\v{s}}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
% \author{I.~Komarov}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{T.~Konno}\affiliation{Kitasato University, Sagamihara 252-0373} % Kitasato
  \author{A.~Korobov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{S.~Korpar}\affiliation{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{E.~Kovalenko}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{P.~Kri\v{z}an}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{R.~Kroeger}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{J.-F.~Krohn}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{P.~Krokovny}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{T.~Kuhr}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
  \author{M.~Kumar}\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017} % MNIT
  \author{R.~Kumar}\affiliation{Punjab Agricultural University, Ludhiana 141004} % Punjab
%% changed per required on bn1547_ml:0185  \author{K.~Kumara}\affiliation{Wayne State University, Detroit, Michigan 48202} % WayneState
  \author{K.~Kumara}\affiliation{University of Mississippi, University, Mississippi 38677} % Mississippi
% \author{T.~Kumita}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
% \author{E.~Kurihara}\affiliation{Chiba University, Chiba 263-8522} % Chiba
  \author{A.~Kuzmin}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
% \author{P.~Kvasni\v{c}ka}\affiliation{Faculty of Mathematics and Physics, Charles University, 121 16 Prague} % Charles
  \author{Y.-J.~Kwon}\affiliation{Yonsei University, Seoul 03722} % Yonsei
  \author{Y.-T.~Lai}\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583} % IPMU
% \author{K.~Lalwani}\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017} % MNIT
  \author{T.~Lam}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{J.~S.~Lange}\affiliation{Justus-Liebig-Universit\"at Gie\ss{}en, 35392 Gie\ss{}en} % Giessen
  \author{M.~Laurenza}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma}\affiliation{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma} % RomaTre
% \author{I.~S.~Lee}\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763} % Hanyang
% \author{J.~K.~Lee}\affiliation{Seoul National University, Seoul 08826} % Seoul
  \author{S.~C.~Lee}\affiliation{Kyungpook National University, Daegu 41566} % Kyungpook
% \author{D.~Levit}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{P.~Lewis}\affiliation{University of Bonn, 53115 Bonn} % Bonn
% \author{C.~H.~Li}\affiliation{Liaoning Normal University, Dalian 116029} % LNNU
  \author{J.~Li}\affiliation{Kyungpook National University, Daegu 41566} % Kyungpook
%  \author{L.~K.~Li}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{S.~X.~Li}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
  \author{Y.~Li}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
  \author{Y.~B.~Li}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{Z.~Li}\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026} % USTC
  \author{L.~Li~Gioi}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{J.~Libby}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
  \author{K.~Lieret}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{Z.~Liptak}\affiliation{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530} % Hiroshima
  \author{D.~Liventsev}\affiliation{Wayne State University, Detroit, Michigan 48202}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % WayneState
% \author{A.~Loos}\affiliation{University of South Carolina, Columbia, South Carolina 29208} % SouthCarolina
% \author{T.~Luo}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{J.~MacNaughton}\affiliation{University of Miyazaki, Miyazaki 889-2192} % NPC
  \author{A.~Martini}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{M.~Masuda}\affiliation{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047} % NPC
  \author{T.~Matsuda}\affiliation{University of Miyazaki, Miyazaki 889-2192} % NPC
  \author{D.~Matvienko}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
  \author{S.~K.~Maurya}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
% \author{J.~T.~McNeil}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
  \author{F.~Meier}\affiliation{Duke University, Durham, North Carolina 27708} % Duke
  \author{M.~Merola}\affiliation{INFN - Sezione di Napoli, I-80126 Napoli}\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli} % Napoli
  \author{F.~Metzner}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
  \author{K.~Miyabayashi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{Nara Women's University, Nara 630-8506} % Nara
% \author{H.~Miyake}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Miyata}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{R.~Mizuk}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{National Research University Higher School of Economics, Moscow 101000} % Lebedev
  \author{G.~B.~Mohanty}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{S.~Mohanty}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005}\affiliation{Utkal University, Bhubaneswar 751004} % Tata
  \author{H.~K.~Moon}\affiliation{Korea University, Seoul 02841} % Korea
% \author{T.~J.~Moon}\affiliation{Seoul National University, Seoul 08826} % Seoul
% \author{H.-G.~Moser}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{M.~Mrvar}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
% \author{T.~M\"uller}\affiliation{Institut f\"ur Experimentelle Teilchenphysik, Karlsruher Institut f\"ur Technologie, 76131 Karlsruhe} % Karlsruhe
% \author{R.~Mussa}\affiliation{INFN - Sezione di Torino, I-10125 Torino} % Torino
% \author{I.~Nakamura}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{K.~R.~Nakamura}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{E.~Nakano}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
% \author{T.~Nakano}\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047} % NPC
  \author{M.~Nakao}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Nakayama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{H.~Nakazawa}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{D.~Narwal}\affiliation{Indian Institute of Technology Guwahati, Assam 781039} % IITG
  \author{Z.~Natkaniec}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{A.~Natochii}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{L.~Nayak}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{M.~Nayak}\affiliation{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978} % TelAviv
% \author{C.~Niebuhr}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{M.~Niiyama}\affiliation{Kyoto Sangyo University, Kyoto 603-8555} % NPC
  \author{N.~K.~Nisar}\affiliation{Brookhaven National Laboratory, Upton, New York 11973} % BNL
  \author{S.~Nishida}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{K.~Nishimura}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{K.~Ogawa}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{S.~Ogawa}\affiliation{Toho University, Funabashi 274-8510} % Toho
% \author{S.~Okuno}\affiliation{Kanagawa University, Yokohama 221-8686} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{Chung-Ang University, Seoul 06974} % CAU
  \author{H.~Ono}\affiliation{Nippon Dental University, Niigata 951-8580}\affiliation{Niigata University, Niigata 950-2181} % NihonDental
% \author{Y.~Onuki}\affiliation{Department of Physics, University of Tokyo, Tokyo 113-0033} % Tokyo
  \author{P.~Oskin}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{H.~Ozaki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{P.~Pakhlov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{National Research University Higher School of Economics, Moscow 101000} % Lebedev
  \author{G.~Pakhlova}\affiliation{National Research University Higher School of Economics, Moscow 101000}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % HSE
% \author{T.~Pang}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
  \author{S.~Pardi}\affiliation{INFN - Sezione di Napoli, I-80126 Napoli} % Napoli
  \author{H.~Park}\affiliation{Kyungpook National University, Daegu 41566} % Kyungpook
  \author{S.-H.~Park}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{A.~Passeri}\affiliation{INFN - Sezione di Roma Tre, I-00146 Roma} % RomaTre
  \author{S.~Patra}\affiliation{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306} % IISERM
  \author{S.~Paul}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % TUM
 \author{T.~K.~Pedlar}\affiliation{Luther College, Decorah, Iowa 52101} % Luther
  \author{R.~Pestotnik}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{L.~E.~Piilonen}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
  \author{T.~Podobnik}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{V.~Popov}\affiliation{National Research University Higher School of Economics, Moscow 101000} % HSE
% \author{S.~Prell}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
  \author{E.~Prencipe}\affiliation{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich} % Juelich
  \author{M.~T.~Prim}\affiliation{University of Bonn, 53115 Bonn} % Bonn
% \author{M.~V.~Purohit}\affiliation{Okinawa Institute of Science and Technology, Okinawa 904-0495} % OIST
% \author{A.~Rabusov}\affiliation{Department of Physics, Technische Universit\"at M\"unchen, 85748 Garching} % TUM
% \author{P.~K.~Resmi}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
% \author{M.~Ritter}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{M.~R\"{o}hrken}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{A.~Rostomyan}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{N.~Rout}\affiliation{Indian Institute of Technology Madras, Chennai 600036} % IITM
% \author{M.~Rozanska}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{G.~Russo}\affiliation{Universit\`{a} di Napoli Federico II, I-80126 Napoli} % Napoli
  \author{D.~Sahoo}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
% \author{Y.~Sakai}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{M.~Salehi}\affiliation{University of Malaya, 50603 Kuala Lumpur}\affiliation{Ludwig Maximilians University, 80539 Munich} % Malaya
  \author{S.~Sandilya}\affiliation{Indian Institute of Technology Hyderabad, Telangana 502285} % IITH
  \author{A.~Sangal}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
  \author{L.~Santelj}\affiliation{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
% \author{T.~Sanuki}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
% \author{Y.~Sato}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{V.~Savinov}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
% \author{P.~Schmolz}\affiliation{Ludwig Maximilians University, 80539 Munich} % LMU
% \author{O.~Schneider}\affiliation{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015} % Lausanne
  \author{G.~Schnell}\affiliation{Department of Physics, University of the Basque Country UPV/EHU, 48080 Bilbao}\affiliation{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao} % Bilbao
% \author{M.~Schram}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
  \author{J.~Schueler}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{C.~Schwanda}\affiliation{Institute of High Energy Physics, Vienna 1050} % Vienna
%  \author{A.~J.~Schwartz}\affiliation{University of Cincinnati, Cincinnati, Ohio 45221} % Cincinnati
% \author{B.~Schwenker}\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen} % Goettingen
% \author{R.~Seidl}\affiliation{RIKEN BNL Research Center, Upton, New York 11973} % RIKEN
  \author{Y.~Seino}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{K.~Senyo}\affiliation{Yamagata University, Yamagata 990-8560} % Yamagata
% \author{O.~Seon}\affiliation{Graduate School of Science, Nagoya University, Nagoya 464-8602} % Nagoya
% \author{I.~S.~Seong}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{M.~E.~Sevior}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{M.~Shapkin}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
  \author{C.~Sharma}\affiliation{Malaviya National Institute of Technology Jaipur, Jaipur 302017} % MNIT
% \author{V.~Shebalin}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
% \author{C.~P.~Shen}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{H.~Shibuya}\affiliation{Toho University, Funabashi 274-8510} % Toho
  \author{J.-G.~Shiu}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
% \author{B.~Shwartz}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{A.~Sibidanov}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
  \author{F.~Simon}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
  \author{J.~B.~Singh}\altaffiliation[also at ]{University of Petroleum and Energy Studies, Dehradun 248007}\affiliation{Panjab University, Chandigarh 160014} % Panjab
% \author{R.~Sinha}\affiliation{Institute of Mathematical Sciences, Chennai 600113} % IMSC
% \author{K.~Smith}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{A.~Sokolov}\affiliation{Institute for High Energy Physics, Protvino 142281} % Protvino
% \author{Y.~Soloviev}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{E.~Solovieva}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{S.~Stani\v{c}}\affiliation{University of Nova Gorica, 5000 Nova Gorica} % NovaGorica
  \author{M.~Stari\v{c}}\affiliation{J. Stefan Institute, 1000 Ljubljana} % Ljubljana
  \author{Z.~S.~Stottler}\affiliation{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061} % VPI
% \author{J.~F.~Strube}\affiliation{Pacific Northwest National Laboratory, Richland, Washington 99352} % PNNL
% \author{J.~Stypula}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
  \author{M.~Sumihama}\affiliation{Gifu University, Gifu 501-1193}\affiliation{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047} % NPC
% \author{K.~Sumisawa}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{T.~Sumiyoshi}\affiliation{Tokyo Metropolitan University, Tokyo 192-0397} % TMU
% \author{W.~Sutcliffe}\affiliation{University of Bonn, 53115 Bonn} % Bonn
% \author{S.~Y.~Suzuki}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
  \author{M.~Takizawa}\affiliation{Showa Pharmaceutical University, Tokyo 194-8543}\affiliation{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198} % NPC
  \author{U.~Tamponi}\affiliation{INFN - Sezione di Torino, I-10125 Torino} % Torino
% \author{S.~Tanaka}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{K.~Tanida}\affiliation{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195} % NPC
% \author{N.~Taniguchi}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{Y.~Tao}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
% \author{G.~N.~Taylor}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{F.~Tenchini}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
% \author{Y.~Teramoto}\affiliation{Osaka City University, Osaka 558-8585} % OsakaCity
% \author{A.~Thampi}\affiliation{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich} % Juelich
% \author{R.~Tiwary}\affiliation{Tata Institute of Fundamental Research, Mumbai 400005} % Tata
% \author{K.~Trabelsi}\affiliation{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay} % IJCLab
% \author{T.~Tsuboyama}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{M.~Uchida}\affiliation{Tokyo Institute of Technology, Tokyo 152-8550} % NPC
% \author{I.~Ueda}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{S.~Uehara}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{T.~Uglov}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991}\affiliation{National Research University Higher School of Economics, Moscow 101000} % Lebedev
% \author{Y.~Unno}\affiliation{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763} % Hanyang
  \author{K.~Uno}\affiliation{Niigata University, Niigata 950-2181} % Niigata
  \author{S.~Uno}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
% \author{P.~Urquijo}\affiliation{School of Physics, University of Melbourne, Victoria 3010} % Melbourne
  \author{Y.~Ushiroda}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}\affiliation{SOKENDAI (The Graduate University for Advanced Studies), Hayama 240-0193} % KEK
  \author{Y.~Usov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{S.~E.~Vahsen}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{R.~Van~Tonder}\affiliation{University of Bonn, 53115 Bonn} % Bonn
  \author{G.~Varner}\affiliation{University of Hawaii, Honolulu, Hawaii 96822} % Hawaii
  \author{K.~E.~Varvell}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{A.~Vinokurova}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
% \author{V.~Vorobyev}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % BINP
  \author{A.~Vossen}\affiliation{Duke University, Durham, North Carolina 27708} % Duke
  \author{E.~Waheed}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{B.~Wang}\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen} % MPI
% \author{C.~H.~Wang}\affiliation{National United University, Miao Li 36003} % NUU
% \author{D.~Wang}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
  \author{E.~Wang}\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} % Pittsburgh
  \author{M.-Z.~Wang}\affiliation{Department of Physics, National Taiwan University, Taipei 10617} % Taiwan
  \author{X.~L.~Wang}\affiliation{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443} % Fudan
% \author{M.~Watanabe}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{Y.~Watanabe}\affiliation{Kanagawa University, Yokohama 221-8686} % Kanagawa
  \author{S.~Watanuki}\affiliation{Yonsei University, Seoul 03722} % Yonsei
% \author{S.~Wehle}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{O.~Werbycka}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{E.~Widmann}\affiliation{Stefan Meyer Institute for Subatomic Physics, Vienna 1090} % Vienna
  \author{J.~Wiechczynski}\affiliation{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342} % Krakow
% \author{E.~Won}\affiliation{Korea University, Seoul 02841} % Korea
% \author{X.~Xu}\affiliation{Soochow University, Suzhou 215006} % Soochow
  \author{B.~D.~Yabsley}\affiliation{School of Physics, University of Sydney, New South Wales 2006} % Sydney
% \author{S.~Yamada}\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801} % KEK
% \author{H.~Yamamoto}\affiliation{Department of Physics, Tohoku University, Sendai 980-8578} % Tohoku
  \author{W.~Yan}\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026} % USTC
  \author{S.~B.~Yang}\affiliation{Korea University, Seoul 02841} % Korea
  \author{H.~Ye}\affiliation{Deutsches Elektronen-Synchrotron, 22607 Hamburg} % DESY
  \author{J.~Yelton}\affiliation{University of Florida, Gainesville, Florida 32611} % Florida
  \author{J.~H.~Yin}\affiliation{Korea University, Seoul 02841} % Korea
% \author{Y.~Yook}\affiliation{Yonsei University, Seoul 03722} % Yonsei
  \author{C.~Z.~Yuan}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
% \author{Y.~Yusa}\affiliation{Niigata University, Niigata 950-2181} % Niigata
% \author{Y.~Zhai}\affiliation{Iowa State University, Ames, Iowa 50011} % ISU
% \author{J.~Zhang}\affiliation{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049} % IHEP
  \author{Z.~P.~Zhang}\affiliation{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026} % USTC
  \author{V.~Zhilich}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
  \author{V.~Zhukova}\affiliation{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991} % Lebedev
% \author{V.~Zhulanov}\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}\affiliation{Novosibirsk State University, Novosibirsk 630090} % BINP
\collaboration{The Belle Collaboration}

